IMaT: Unsupervised Text Attribute Transfer via Iterative Matching and Translation

Text attribute transfer aims to automatically rewrite sentences such that they possess certain linguistic attributes, while simultaneously preserving their semantic content. This task remains challenging due to a lack of supervised parallel data. Existing approaches try to explicitly disentangle content and attribute information, but this is difficult and often results in poor content-preservation and ungrammaticality. In contrast, we propose a simpler approach, Iterative Matching and Translation (IMaT), which: (1) constructs a pseudo-parallel corpus by aligning a subset of semantically similar sentences from the source and the target corpora; (2) applies a standard sequence-to-sequence model to learn the attribute transfer; (3) iteratively improves the learned transfer function by refining imperfections in the alignment. In sentiment modification and formality transfer tasks, our method outperforms complex state-of-the-art systems by a large margin. As an auxiliary contribution, we produce a publicly-available test set with human-generated transfer references.

==> sections/method_acl.tex <==
\section{Method}
\label{sec:method}



% \subsection{Problem Definition}
Given two corpora $X=\{x_1,\cdots,x_n\}$ of style $s_1$ and $Y=\{y_1,\cdots,y_m\}$ of style $s_2$, the style transfer task requires the model to transfer a sentence $x_i$ from style $s_1$ to style $s_2$, while preserving its content. 
Style transfer can be tackled using standard machine translation techniques in a scenario where each sentence in $Y$ is a rewritten version of a source sentence in $X$.  However, in most style transfer tasks, $X$ and $Y$ are not parallel, thus the system has no access to any rewrite in the training data, and the appropriate alignments have to be learned in an unsupervised fashion.

% \myworries{I recommend to remove the OT stuff from here (you may write a short paragraph of it in the related work, when you situate our model: you can say that we also rely on OT, but really couple of sentences). It is not giving any insight and it is mostly adding noise that confuses the reader.}
% \todo[size=\small, color=red!50]{I kind of agree with the current smooth flow. Let's see what Jonas thinks.}

%\paragraph{Relation to Optimal Transport (OT)} One way to look at style transfer is through the lens of Optimal Transport \cite{villani2008optimal}, where the cost of transporting one sentence to another is quantified by the semantic shift. Under this perspective, style transfer seeks out the most cost-efficient transport map $M$ that turns the underlying distribution of the source sentences $\mathbb{P}_{X}$ into the distribution of the target sentences $\mathbb{P}_{Y}$. % (satisfying the constraint ${M(x) \sim \mathbb{P}_{X_2}}$ for ${x \sim \mathbb{P}_{X_1}}$). However, formulating style transfer as standard OT is not entirely satisfactory because the latter distributional constraint is overly strong, forcing $M$ to produce substantial content-shifts for some source sentences if the target distribution differs quite a bit from the source (particularly if there are differences in not only style, but also in content, which is typically the case for non-parallel corpora). 
%A desirable style transfer function that imposes hard limits on content shifts may require a relaxation of the OT distributional constraints.  In this case, it is sufficient to train the transport map $M$ on source-target pairs with high content similarity. % (which we bound in this work through our combination of the measures \myworries{TODO: Sim and NounRetention}). 
%While only training $M$ on a subset of the supports of ${\mathbb{P}_{X}, \mathbb{P}_{Y}}$ %(for which the similarity-threshold is met) 
%will violate the OT-condition ${M(\mathbb{P}_{X}) =  \mathbb{P}_{Y}}$, sentences generated from $M$ should nonetheless look like they come from the target corpus distribution. % (with ample probability under $\mathbb{P}_{X_2}$), since our method selects real sentences from  $X_2$ as the targets of $M$ during training. 
%%%%% THIS IS INTERESTING, BUT SHOULD GO IN THE METHOD %%%%%
%In our iterative model, we gradually expand the sentence-pairs used to train $M^{(t)}$, therefore exposing $M^{(t)}$ to increasingly large portions of the $\mathbb{P}_{X_1},\mathbb{P}_{X_2}$, and encouraging the final map $M^{(T)}$ to reduce the distance between $M^{(T)}(\mathbb{P}_{X_1})$ and $\mathbb{P}_{X_2}$.

\begin{figure*}[t]
    \small
    \centering
    \includegraphics[width= \textwidth]{img/method.png}
    \caption{Iterative process of the algorithm to transfer the style from positive to negative reviews. 
    %(Step 1) We construct pseudo pairs through semantic matching of sentence embeddings. 
    %(Step 2) We transfer the sentence by iteratively translating and matching.
    }
    \label{fig:method}
\end{figure*}




\subsection{Iterative Matching and Translation}
Two large mono-style corpora potentially contain a large number of sentence pairs $(x,y)$ with similar content. Based on this assumption, we propose an iterative matching and translation algorithm composed of three steps: (1) identification of pseudo-pairs by matching sentences in the non-parallel data with an unsupervised similarity function; (2) training a Seq2Seq machine translation model with attention over the pseudo-pairs to generate transfer candidates; and finally, (3) feeding the new transfer candidates to (1), to identify more accurate pseudo-pairs. This refinement-like procedure is repeated until convergence. Specifically, we initially construct a pseudo-parallel corpus by searching for the nearest neighbor sentences in the corpora $X$ and $Y$. We then use the identified matches to bootstrap the iterative process $T$, in which every iteration $t$ consists of (a) training a machine translation model $M^{(t)}$ over the matches to generate new transfer candidates $\hat Y$; (b) retrieving from the target corpus $Y$ the nearest neighbor sentences of the generated candidates $\hat Y$; and (c) re-pairing $X$ with $\hat Y$ as new training data for the translation model in subsequent iterations. This iterative scheme is illustrated in Figure~\ref{fig:overview}. The method is formalized in Algorithm \ref{alg:transfer} and described in details below. %\myworries{In the Figure, I cannot see the growth of training examples (Do we still use all sentences from previous iterations or they are not used anymore? Clarify this!). You may want to represent this memory, as it is relevant. }
%\todo[size=\small, color=red!50]{Only the ``best candidate'' is updated. Afterwards, the best candidate is matched towards ``target corpus''. No other memory is kept.}
%\myworries{Note that above I changed the non-capitalized to capitalized letters (e.g. y hat to Y hat): if you prefer to talk about single cases at a time, get back to the previous format, yet keeping this sentence structure.}
%\todo[size=\small, color=red!50]{Thanks for changing the captalization. I think the current expression is clearer.}
 
\paragraph{(Step 1) Matching.} The iterative training scheme is enabled by the initial, unsupervised, matching of corpora $X$ and $Y$. We construct a large pseudo-parallel corpus $\hat Y^{(0)}$ by pairing every $x\in X$ with a sentence $\hat y$ from $Y$. We identify the pseudo target $\hat y$ by selecting the highest cosine similarity to the unsupervised sentence embedding of $x$. In later iterations, this matching process is repeated between the new pseudo-parallel corpus $\hat Y^{(t)}$ and the target corpus $Y$, where $t$ is the number of iterations. 
% \myworries{Instead of "the new pseudo-parallel corpus $Y$" should not it be "the new pseudo-parallel corpus $Y^{0,1,...t-1}$" or $Y^{t-1}$?}
%\myworries{The new pseudoparallel corpus is composed by $\hat Y^{(0)}$, $\hat Y^{(1)}$, $\hat Y^{(2)}$...? If yes, make sure you explain it and also to use $\hat Y^{(t)}, t=0$ in the first occurrence of $\hat Y^{(0)}$ above.} \note{I tried this and it looks a bit tedious to use $\hat Y^{(t)}, t=0$. How do you like putting the clarification in the green part?}

\paragraph{(Step 2) Translation.} To refine the initial pseudo-parallel corpus, a Seq2Seq machine translation model with attention is trained from scratch. In the iterative process, this translation model plays a denoising role. The pseudo-parallel corpus, initially constructed by extracting the most similar sentence pairs, contains erroneous pseudo-pairs that are similar in trivial ways. For instance, the sentence ``Best \textit{pizza} ever ever'' was initially matched with ``Best \textit{burrito} ever ever'' (Figure~\ref{fig:method}). 

The critical function of the translation model is to capture only relevant and frequent patterns, while ignoring the randomly occurring noise. This is possible because the model takes into consideration the whole pseudo-parallel corpus. This is shown in the sentence (A) of Figure~\ref{fig:method}, where the ``burrito'' was immediately turned into ``pizza'' after the first translation.

\paragraph{(Step 3) Iterative Refinement.} The translation model may also generate divergent outputs. In each iteration $t$, it is therefore important to implement a check-and-update process, which ensures that $\hat Y^{(t)}$ is updated only if the newly generated examples are better than the previous ones. This is done by calculating which version minimizes the transportation cost from the source corpus $X$ to the pseudo-parallel corpus $\hat Y^{(t)}$. Specifically, we consider the total transportation cost as the sum of Word Mover Distance \cite{huang2016supervised} of each source sentence and its pseudo target $(x, \hat y')$. In the following iteration $t + 1$, a new translation model is trained over the updated $(X, \hat Y^{(t)})$. This process keeps refining the pseudo-parallel corpus until a nearly parallel corpus is obtained.

%\newdelete{In each iteration $t$, in order to avoid updating the pseudo-parallel corpus with divergent generated outputs, a check routine is performed before updating}
%\newadd{The outputs of the translation model provides more candidates of pseudo pairs. Thus, we perform a check-and-update process to refine} the pseudo-parallel corpus $\hat Y^{(t)}$ with the these new outputs, and based on the updated corpus, we repeat (Step 1) matching and (Step 2) translation. 
%\newadd{The update of a pseudo target sentence in $\hat Y^{(t)}$ with the newly generated one happens only if the update minimizes the transportation cost from the source corpus $X$ to the pseudo-parallel corpus $\hat Y^{(t)}$. Specifically, we consider the total transportation cost as the sum of Word Mover Distance of each source sentence and its pseudo target $(x, \hat y')$. Therefore, the newest pseudo-parallel corpus $\hat Y^{(t)}$ consists of all pseudo target sentences that have the so-far lowest transportation cost from $X$.} \myworries{I have modified the paragraph Step3 to show that OT is helpful to decide whether updating or not and avoid divergence. Short and punchy. Double check it is correct}\note{The green sentence ``The update of a pseudo target...'' may look a bit long and confusing to a first-time reader.}

%\newadd{The intuition behind the iterative process is that as long as the initial pseuo-parallel corpus provides some information to the translation model $M^{(1)}$, the translation model will gain the major trend of style transfer and, by mapping a large corpus into feature space, it learns a cleaner mapping of source to target, thus acting as a denoiser. At the same time, as the generated sentence provides more noiseless pseudo targets, it provides good foundation for better style translation at the next iteration, and so on so forth.} \myworries{This is redundant. I don't like it. It is written already in the paragraph before: The critical function of the translation model.........}

%\myworries{Y is forgotten forever or it is still used during the following iterations?} \note{See the green text in (Step 1). $Y$ is used in every iterations of matching} \newdelete{This process keeps refining the pseudo-parallel corpus until a nearly parallel corpus is obtained.}{: No need to mention the good performance}

%\myworries{If you have not added any info about OT in the related work, you can write two lines here, very shortly: just mention it in function of the method, without giving other info that are not relevant...}
%\myworries{explain why there may be divergence}

%\newdelete{In order to prevent this process from divergence,  we align our iterative refinement process to the target of Optimal Transport, and minimize the transportation cost from the source corpus $X$ to the pseudo-parallel corpus $\hat Y^{(t)}$ in each iteration. To evaluate the transportation cost of $(x, \hat y)$, we adopt Word Mover Distance (WMD) \cite{huang2016supervised}, which represents the minimum amount of distance that the embedded words of one sentence need to ``travel'' to reach the embedded words of another sentence. The pseudo-parallel corpus is updated only if the transportation cost of $(x, \hat y')$ is lower than that of the existent $(x, \hat y)$. In this way, we optimize the transportation cost of $X$ to $\hat Y^{(t)}$ at each iteration.}
%\myworries{clean up this paragraph, it is a bit unclear and unmotivated}

Two possible trends of iterative outputs are illustrated in Figure~\ref{fig:method}. Sentence (A),  ``Best pizza ever ever'', is not further refined after Iteration 2, because it matched ``Worst pizza ever ever'' with the lowest possible transportation cost. Sentence (B), ``I will return often'', instead, keeps updating throughout the iterations. In order to minimize the transportation cost, sentence (B) changes from ``I will probably return'' to ``I won't return!'', and eventually to ``I will not return!''. The refinement process continues until the percentage of the sentences that are updated in $\hat Y^{(t)}$ by minimizing the transportation cost drops to a negligible value. 
% \myworries{what is update rate? clarify it}

\input{sections/element/algo.tex}









==> sections/old_tex/ori_related.tex <==
% Text style transfer has recently become an active research area~\citep{shen2017style,fu2017style,li2018delete,prabhumoye2018style}.  A lack of parallel data and special texture-features found in images has forced current approaches to use either: inference modules to disentangle style from content in a learned latent representation, or manually-specified heuristics to substitute weakly referential words from the source to the target style.

% \subsection{Text Style Transfer}
% \paragraph{Latent Representation Learning} 
Many existing approaches in text style transfer aim to infer useful latent-variables that facilitate style translation \cite{mueller2017sequence, fu2017style}. \citet{shen2017style}, for example, assume a shared latent content distribution across different text corpora and propose a cross-aligned auto-encoder with adversarial training to discriminate style and content. 
% \citet{fu2017style} use multiple decoder to generate texts of each style. 
% \citet{prabhumoye2018style} ground the latent representation of a sentence in a language translation model to help to preserve its meaning and to reduce the stylistic properties. 
Despite the complexity of these models and their related training difficulties \cite{salimans2016improved, arjovsky2017towards, bousmalis2017unsupervised}, empirically they cannot effectively flip the style without tempering the content or producing ungrammatical sentences. Their outputs are in fact judged as low-quality by human raters.

% \paragraph{Rule-Based Text Manipulation}
Noticing the limitations of GANs, \citet{li2018delete} propose a simple heuristic approach. They first identify phrases with a strong attribute, and then they replace them with phrases of the opposite attribute, training a neural model to combine them in a natural way. This method outperforms the adversarial approaches, but it produces sentences flawed with grammatical errors, as it can be seen in Table~\ref{table:example1}. 

% \paragraph{Style Back-Translation}

In the attempt to improve content preservation and fluency, later works proposed the back-translation objective, that is back-translating the transferred sentences to the source style and comparing them with the original sentences \cite{santos2018fighting,logeswaran2018content,subramanian2018multiple,prabhumoye2018style}. This technique exposes the model to a pseudo-supervised setting \cite{subramanian2018multiple}.


% \paragraph{Pseudo-Parallel Pairs}
% \subsection{Pseudo-Pairing in NMT}

Our proposal also relates to early work on comparable  corpora  for  Statistical  Machine  Translation   (SMT) systems~\cite{fung1998ir,munteanu2004improved,smith2010extracting}, which incrementally trained on pseudo-parallel pairs. This approach was further applied in recent years in the area of unsupervised Neural Machine Translation (NMT)~\citep{conneau2017word,lample2017unsupervised,artetxe2017unsupervised}, which exploits back-translation to ensure that generated sentences can be turned back to the source. Our matching mechanism differs from this in that the pseudo-pairs are always real sentences coming from a non-parallel corpus, and our approach only requires a single translation model rather than two.

%\myworries{This is the most important paragraph to situate our model with respect to the related work. Write it very well. Currently it is super ugly and unclear. Do not use "also relates to early work..." if you have not previously specified that previous works related to it. Do not assume the reader knows it.}
\todo{Here is the new edit}


==> sections/sketch.tex <==
\section{Method}
\label{sec:method}



% \subsection{Problem Definition}
Given two corpora $X=\{x_1,\cdots,x_n\}$ of style $s_1$ and $Y=\{y_1,\cdots,y_m\}$ of style $s_2$, the task consists of learning a model that takes a sentence $x_i$ from style $s_1$ and transfers it into style $s_2$, while preserving its content. 
Style transfer can be tackled using standard machine translation techniques in a scenario where each sentence in $Y$ is a rewritten version of a source sentence in $X$.  However, in most style transfer tasks, $X$ and $Y$ are not parallel, thus the system has no access to any rewrite in the training data, and the appropriate alignments have to be learned in an unsupervised fashion.

\paragraph{Relation to Optimal Transport (OT)} One way to look at style transfer is through the lens of Optimal Transport \cite{villani2008optimal}, where the cost of transporting one sentence to another is quantified by the semantic shift. Under this perspective, style transfer seeks out the most cost-efficient transport map $M$ that turns the underlying distribution of the source sentences $\mathbb{P}_{X}$ into the distribution of the target sentences $\mathbb{P}_{Y}$. % (satisfying the constraint ${M(x) \sim \mathbb{P}_{X_2}}$ for ${x \sim \mathbb{P}_{X_1}}$). However, formulating style transfer as standard OT is not entirely satisfactory because the latter distributional constraint is overly strong, forcing $M$ to produce substantial content-shifts for some source sentences if the target distribution differs quite a bit from the source (particularly if there are differences in not only style, but also in content, which is typically the case for non-parallel corpora). 
A desirable style transfer function that imposes hard limits on content shifts may require a relaxation of the OT distributional constraints.  In this case, it is sufficient to train the transport map $M$ on source-target pairs with high content similarity. % (which we bound in this work through our combination of the measures \myworries{TODO: Sim and NounRetention}). 
While only training $M$ on a subset of the supports of ${\mathbb{P}_{X}, \mathbb{P}_{Y}}$ %(for which the similarity-threshold is met) 
will violate the OT-condition ${M(\mathbb{P}_{X}) =  \mathbb{P}_{Y}}$, sentences generated from $M$ should nonetheless look like they come from the target corpus distribution. % (with ample probability under $\mathbb{P}_{X_2}$), since our method selects real sentences from  $X_2$ as the targets of $M$ during training. 
%%%%% THIS IS INTERESTING, BUT SHOULD GO IN THE METHOD %%%%%
%In our iterative model, we gradually expand the sentence-pairs used to train $M^{(t)}$, therefore exposing $M^{(t)}$ to increasingly large portions of the $\mathbb{P}_{X_1},\mathbb{P}_{X_2}$, and encouraging the final map $M^{(T)}$ to reduce the distance between $M^{(T)}(\mathbb{P}_{X_1})$ and $\mathbb{P}_{X_2}$.

\begin{figure*}[t]
    \small
    \centering
    \includegraphics[width= \textwidth]{img/method.png}
    \caption{Iterative process of our algorithm to transfer the style from positive to negative reviews. 
    %(Step 1) We construct pseudo pairs through semantic matching of sentence embeddings. 
    %(Step 2) We transfer the sentence by iteratively translating and matching.
    }
    \label{fig:method}
\end{figure*}


\iffalse
An alternative way to formalize the style transfer task is through the lens of optimal transport \cite{Villani}. Under this perspective, style transfer seeks the probabilistic transport map $M^*$ between sentences that solves: ${\min_{M} \ \mathbb{E}_{x \sim \mathbb{P}_{X_1}} \mathbb{E}_{x' \sim M(x)} \text{Cost}(x,x')}$ s.t.\ ${M(x) \sim \mathbb{P}_{X_2}}$ for ${x \sim \mathbb{P}_{X_1}}$. Here, $\mathbb{P}_{X_1}$ and $\mathbb{P}_{X_2}$ respectively denote the underlying distribution of source and target sentences, and the cost of transporting one sentence to another $\text{Cost}(x,x')$
is quantified by the shift in content/semantics (which we quantify in this work by combining the measures Sim and NounRetention).

However, reformulating style transfer as a standard Optimal Transport problem is not entirely satisfactory  because the distributional constraint $M(\mathbb{P}_{X_1}) = \mathbb{P}_{X_2}$ is overly strong, forcing $M$ to  

\bigskip
(= $C - \text{Sim}(x_1, x_2)$ for some content-similarity-measure Sim whose maximal value is $C$)
\fi
% End of Jonas addition.

\subsection{Iterative Matching and Translation}
Two large mono-style corpora potentially contain a large number of sentence pairs $(x,y)$ of different styles but similar content. Based on this property, we propose an iterative matching and translation algorithm composed of three steps, namely (1) identification of pseudo-pairs by matching sentences in the non-parallel data with an unsupervised similarity function; (2) training a sequence-to-sequence machine translation model with attention over the pseudo-pairs to generate transfer candidates; and finally, (3) feeding the new transfer candidates to (1), searching for more accurate pseudo-pairs, until convergence. %initially identifying high quality alignments between a subset of the source-target pairs whose translation should confidently preserve content. From such matches, we can iteratively generate synthetic transfers through a machine translation algorithm and search for additional source-target pairs, in a refinement-like procedure. 
{Specifically, we first construct a pseudo-parallel corpus by searching for the nearest neighbor between corpus $X$ and $Y$. This bootstraps the following process: For each iteration $t$, we train a machine translation model $M^{(t)}$ to generate new transfer candidates $\hat y$. We then retrieve the nearest neighbor of the new transfer candidate from the target corpus $Y$, and re-pair $x$ with $\hat y$ as the training data for the translation model of the subsequent iteration. The refinement through this iterative scheme is illustrated in Figure~\ref{fig:overview}. The method is formalized in Algorithm \ref{alg:transfer} and described in details below.} 
 


\iffalse
We revise our similarity measure accordingly:
\begin{align}
\text{Sim}(x_1,x_2)=
\begin{cases}
\text{tf-idf}(x_1,x_2), & l_1/r \leqslant l_2 \leqslant r\cdot l_1\\
0, & \text{o.w.}
\end{cases}
\end{align}
where $l_1,l_2$ are the lengths of $x_1,x_2$ respectively. In our experiments we set $r=1.5$.
\fi


\paragraph{(Step 1) Matching.} The iterative training scheme is enabled by the initial, unsupervised matching of corpora $X$ and $Y$. We construct a large pseudo-parallel corpus $\hat Y^{(0)}$ by pairing every $x\in X$ with a sentence $\hat y$ from $Y$. The pseudo target $\hat y$ has the highest cosine similarity to the unsupervised sentence embedding of $x$. In later iterations, this matching process is repeated between the new pseudo-parallel corpus $\hat Y$ and $Y$.

\paragraph{(Step 2) Translation.} To refine the initial pseudo-parallel corpus, we train a sequence-to-sequence machine translation model with attention from scratch. In the iterative process, it plays a denoising role. The pseudo-parallel corpus, initially constructed by extracting the most similar sentence pairs, contains erroneous pseudo-pairs that are similar in some trivial way but not the topic. For instance, the sentence ``Best \textit{pizza} ever ever'' was initially matched with ``Best \textit{burrito} ever ever'' in Figure~\ref{fig:method}. 

The critical function of the translation model is to capture only relevant patterns because it takes into consideration the whole pseudo-parallel corpus. As a result, many erroneous examples are immediately refined by the translation model. As shown in the sentence (A) of Figure~\ref{fig:method}, the ``burrito'' was turned into ``pizza'' after the first translation.

\paragraph{(Step 3) Iterative Refinement.} We update the pseudo-parallel corpus $\hat Y$ by the outputs of the translation model and iteratively repeat (Step 1) matching and (Step 2) translation. At iteration $t$, a new translation model is trained based on the updated $(X, \hat Y^{(t)})$. This process keep refining the pseudo-parallel corpus until a nearly parallel corpus is obtained. 

In order to prevent this process from divergence, we align our iterative refinement process to the target of Optimal Transport, and minimize the transportation cost from the source corpus $X$ to the pseudo-parallel corpus $\hat Y$ in each iteration. To evaluate the transportation cost of $(x, \hat y)$, we adopt Word Mover Distance (WMD) \citep{huanggao2016nips}, which represents the minimum amount of distance that the embedded words of one sentence need to ``travel'' to reach the embedded words of another sentence. The pseudo-parallel corpus is updated only if the transportation cost of $(x, \hat y')$ is lower than that of the existent $(x, \hat y)$. In this way, we optimize the transportation cost of $X$ to $\hat Y$ at each iteration.

Two possible trend of iterative outputs are illustrated in Figure~\ref{fig:method}. Sentence (A)  ``Best pizza ever ever'' stops refinement after Iteration 2, because it already found a match ``Worst pizza ever ever'' with the lowest possible transportation cost. However, sentence (B) ``I will return often'' keeps updating throughout the iterations. In order to minimize the transportation cost, it updates from ``I will probably return'' to ``I won't return!'' and eventually to ``I will not return!'' which has increasingly lower transportation cost. The refinement process continues until the update rate drops to a negligible value.

\input{sections/element/algo.tex}




\iffalse
\subsection{Model}
Our proposed model is based on the prevalence of large single-style corpora (e.g. sentiment, political slant, gender tones, etc.). Therefore, a near-to-perfect match can always be found in the target corpus. The key point is to come up with a model that captures only semantic content and neglects other attributes. 

We denote the $n$th soft alignment as $A_n$, where $A_n$ maps a source sentence $x_i^{({S_0})}$ to a target sentence $x_j^{({S_1})}$. We denote the alignment as $A_n(x_i^{({S_0})}) = x_j^{({S_1})}$. 

\begin{figure}[h!]
  \caption{The Iterative Soft Alignment}
  \centering
  \includegraphics[width=0.5\textwidth]{img/model.png}
\end{figure}
\paragraph{Bootstrapping}
The initial alignment function $A_0$ is
\begin{equation}\label{A_0}
    \argminE_{x_j^{(S_1)} \in D_{S_1}} dist(\cdot{}, x_j^{({S_1})})
\end{equation}
where $dist$ is a distance metric comparing two sequences of words. In our model, we used TF-IDF weighted word overlap.

Then we generate the soft-aligned parallel dataset $\{x_i^{({S_0})}, A_0(x_i^{({S_0})})\}$, where each $(x_i^{({S_0})}, A_0(x_i^{({S_0})}))$ is a pair of sentences. 

\paragraph{Iterative Training}

The final learning algorithm is described in Algorithm 1 and Figure 3.
\begin{figure*}[h!]
  \caption{Illustration of the proposed architecture}
  \centering
  \includegraphics[width=0.6\textwidth]{img/Picture1.png}
\end{figure*}

For each iteration $n$, we first derive a soft-aligned parallel dataset $\{x_i^{({S_0})}, A_0(x_i^{({S_0})})\}$. Then we train a Seq2Seq model $M_{\theta}$ with Attention on the parallel dataset. We use $M_{\theta}(\cdot)$ to generate a target set $\{M_{\theta}(x_i^{({S_0})})\}$. We obtain the new $A_{n+1}$ by 
\begin{equation}\label{A_0}
    A_{n+1}(\cdot) = \argminE_{x_j^{(S_1)} \in D_{S_1}} dist( M_{\theta}(\cdot)  , x_j^{({S_1})})
\end{equation}
where $dist$ is the distance metric between two sequences of words. 

Additionally, in order to reinforce the convergence, we apply a filter which compares the retain rate of keywords in transferred sentences $A_n(x_i^{(S_0)})$ with $A_{n+1}(x_i^{(S_0)})$ for each $i$. Only a generated sentence with higher retain rate of content words are used.  $A_n(x_i^{(S_0)})$ with $A_{n+1}(x_i^{(S_0)})$ for each $i$. We collect a keyword library $\{K\}$ for certain contents. We define the content retain rate $R$ as the F1 score of content keywords in source sentences and those in target sentences. Only the target sentences with higher content retain rate than before are kept. 

We continue this iterative training until the updating rate in the new paired dataset is lower than a threshold $\epsilon$.
\fi




